Transferability Properties of Graph Neural Networks

Graph neural networks (GNNs) are composed of layers consisting of graph convolutions and pointwise nonlinearities. Due to their invariance and stability properties, GNNs are provably successful at learning representations from data supported on moderate-scale graphs. However, they are difficult to learn on large-scale graphs. In this paper, we study the problem of training GNNs on graphs of moderate size and transferring them to large-scale graphs. We use graph limits called graphons to define limit objects for graph filters and GNNs -- graphon filters and graphon neural networks (WNNs) -- which we interpret as generative models for graph filters and GNNs. We then show that graphon filters and WNNs can be approximated by graph filters and GNNs sampled from them on weighted and stochastic graphs. Because the error of these approximations can be upper bounded, by a triangle inequality argument we can further bound the error of transferring a graph filter or a GNN across graphs. Our results show that (i) the transference error decreases with the graph size, and (ii) that graph filters have a transferability-discriminability tradeoff that in GNNs is alleviated by the scattering behavior of the nonlinearity. These findings are demonstrated empirically in a movie recommendation problem and in a decentralized control task.

==> figures/figures/1030/10_filter_convergence.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex


\def \thisplotscale {1.0}
\def \unit {\thisplotscale cm}

\tikzstyle {block blue} = [ block, 
                            thin,
                            minimum width  = 2.8*\unit, 
                            minimum height = 1.3*\unit, 
                            anchor = west,
                            fill = blue!15]

\tikzstyle {block green} = [ block blue, 
                             fill = mygreen!25]

\tikzstyle {block gray} = [ block blue, 
                            fill = black!15]


\def \deltax      {+1.0}
\def \deltaother  {+0.7}

\def \graphfilter   {
                      % \only<2- | handout : 1> 
                       %   {\bie \bbH(\bbS_n) = \sum_{k=1}^{K} \red{h_k} \bbS_n^{k}  \eie}
                        \only<2- | handout : 1> 
                          {\bie \bby_n = \sum_{k=1}^{K} \red{h_k} \bbS_n^{k} \bbx_n \eie}
                    }

\def \graphonfilter {
                       %\only<2-7 | handout : 1> 
                        %  {\bie T_H = \sum_{k=1}^{K} \red{h_k} T_\bbW^{(k)}  \eie}
                        \only<3-  | handout : 1> 
                          {\bie \bby_n = \sum_{k=1}^{K} \red{h_k} T_\bbW^{(k)} X  \eie}
                    }

{\footnotesize

\begin{tikzpicture}[x = 1*\unit, y = 1*\unit]


   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   % GFT chain
   
   % Begin by drawing an empty node for initializing the chain
   \node (T0) [] {};

   % Draw the chain of graph shifts. 
   \os{2-}{\path (T0.east) ++ (\deltax, 0) node (T1) [block green] {\graphfilter};}

   % End by drawing an empty node at the end of the chain
   \path (T1.east) ++ (\deltax, 0) node (T2) [] {};
   
   % Draw the arrows connecting the blocks
   \os{2-}{\path[-stealth, draw] (T0) -- (T1) node [near start, above] {$\bbx_n$};}	
   \os{2-}{\path[-stealth, draw] (T1) -- (T2) node [near end,   above] {$\bby_n$};}	   

   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   % WFT chain
   
   % Begin by drawing an empty node for initializing the chain
   \path (T2.east) ++ (\deltaother, 0) node (B0) [] {};

   % Draw the chain of graph shifts. 
   \os{3-}{\path (B0.east) ++ (\deltax, 0) node (B1) [block blue] {\graphonfilter};}

   % End by drawing an empty node at the end of the chain
   \path (B1.east) ++ (\deltax, 0) node (B2) [] {};
   
   % Draw the arrows connecting the blocks
   \os{3-}{\path[-stealth, draw] (B0) -- (B1) node [near start, above] {$X$};}	
   \os{3-}{\path[-stealth, draw] (B1) -- (B2) node [near end,   above] {$Y$};}	   


\end{tikzpicture}

}

        


==> figures/figures/1030/23_low_pass_lipschitz_filter.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}

\def \frequencyresponse 
     { 0.1*exp(-(1*(x-4.3))^2) 
       + 0.25*exp(-(2*(x-4.5))^2) 
       + 0.37*exp(-(1.3*(x-6.5))^2) 
       + 0.55}
       
\def \flatfrequencyresponse 
     { 0.}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 enlarge x limits = false,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,
             legend pos=north east,
             legend columns=3]
         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=2.1:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\frequencyresponse};
         
\addplot+[samples at = {2.1}, 
          mark=otimes*, 
          mark options={black}]
         {\frequencyresponse};
         
\addplot[ domain=0:2.1, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {2.1}, 
          mark=*, 
          mark options={black, fill=white}]
         {\flatfrequencyresponse};

\end{axis}

\end{tikzpicture}

}



==> figures/figures/1030/26_low_pass_lipschitz_filter_high_eig.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}

\def \frequencyresponse 
     { 0.1*exp(-(1*(x-4.3))^2) 
       + 0.25*exp(-(2*(x-4.5))^2) 
       + 0.37*exp(-(1.3*(x-6.5))^2) 
       + 0.55}
       
\def \flatfrequencyresponse 
     { 0.}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 enlarge x limits = false,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,
             enlarge x limits=false,             					
             legend pos=north east,
             legend columns=3]

\addplot+[samples at = {0.00, 0.02, 0.04, 0.1, 		              
			  0.2, 0.3, 0.45, 0.6, 0.79, 1.03, 1.57}, 
          color = blue!30, 
          ycomb, 
          mark=otimes*, 
          mark options={blue!30}]
         {\frequencyresponse};
         
\addplot+[samples at = {0.04, 0.175, 0.155, 0.34, 0.355, 
              0.66, 0.72, 1.17, 1.4}, 
          color = mygreen!30, 
          ycomb, 
          mark=otimes*, 
          mark options={mygreen!30}]
         {\frequencyresponse};

         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=2.1:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\frequencyresponse};
         
\addplot+[samples at = {2.1}, 
          mark=otimes*, 
          mark options={black}]
         {\frequencyresponse};
         
\addplot[ domain=0:2.1, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {2.1}, 
          mark=*, 
          mark options={black, fill=white}]
         {\flatfrequencyresponse};

%   \addlegendentry{\scriptsize $\bbW$}
%   \addlegendentry{\scriptsize $\bbG_n$}

\end{axis}

\end{tikzpicture}

}



==> figures/figures/1030/43_constant_filter.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}
\def \unit {\thisplotscale cm}
       
\def \flatfrequencyresponse 
     { 0.55}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,
             legend pos=north east,
             legend columns=3]
         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=0:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponse};

\end{axis}

\end{tikzpicture}

}


==> figures/figures/1030/43_high_pass_filter.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}
\def \unit {\thisplotscale cm}
       
\def \flatfrequencyresponse 
     { 0.55}
     
            
\def \flatfrequencyresponsezero 
     { 0.0}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,
             legend pos=north east,
             legend columns=3]
         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=0:2.1, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponse};
         
\addplot[ domain=2.1:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponsezero};
         
\addplot+[samples at = {2.1}, 
          mark=*, 
          mark options={black, fill=white}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {2.1}, 
          mark=*, 
          mark options={black}]
         {\flatfrequencyresponsezero};

\end{axis}

\end{tikzpicture}

}


==> figures/figures/1030/46_constant_filter_graphon_eig.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}
\def \unit {\thisplotscale cm}
       
\def \flatfrequencyresponse 
     { 0.55}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,
             legend pos=north east,
             legend columns=3]

\addplot+[samples at = {0.00, 0.02, 0.04, 0.1, 		              
			  0.2, 0.3, 0.45, 0.6, 0.79, 1.03, 1.57, 
              2.63, 3, 4.24, 5.51, 6.72, 7.6}, 
          color = blue!60, 
          ycomb, 
          mark=otimes*, 
          mark options={blue!60}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {0.04, 0.175, 0.155, 0.34, 0.355, 
              0.66, 0.72, 1.17, 1.4, 2.5, 3.13, 4.13, 
              5.68, 6.87, 7.8}, 
          color = mygreen!60, 
          ycomb, 
          mark=otimes*, 
          mark options={mygreen!60}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=0:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponse};

%   \addlegendentry{\scriptsize $\bbW$}
%   \addlegendentry{\scriptsize $\bbG_n$}

\end{axis}

\end{tikzpicture}

}


==> figures/figures/1030/49_constant_filter_zeroc_graphon_eig.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}
\def \unit {\thisplotscale cm}
       
\def \flatfrequencyresponse 
     { 0.55}
     
\def \flatfrequencyresponsezero 
     { 0.0}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,
             legend pos=north east,
             legend columns=3]

\addplot+[samples at = {0.00, 0.02, 0.04, 0.1, 		              
			  0.2, 0.3, 0.45, 0.6, 0.79, 1.03, 1.57}, 
          color = blue!60, 
          ycomb, 
          mark=otimes*, 
          mark options={blue!60}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {0.04, 0.175, 0.155, 0.34, 0.355, 
              0.66, 0.72, 1.17, 1.4}, 
          color = mygreen!60, 
          ycomb, 
          mark=otimes*, 
          mark options={mygreen!60}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=0:2.1, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {2.1}, 
          mark=*, 
          mark options={black, fill=white}]
         {\flatfrequencyresponse};
         
\addplot[ domain=2.1:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponsezero};
         
\addplot+[samples at = {2.1}, 
          mark=otimes*, 
          mark options={black}]
         {\flatfrequencyresponsezero};

%   \addlegendentry{\scriptsize $\bbW$}
%   \addlegendentry{\scriptsize $\bbG_n$}

\end{axis}

\end{tikzpicture}

}


==> figures/figures/1030/49_high_pass_filter_eig.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}
\def \unit {\thisplotscale cm}
       
\def \flatfrequencyresponse 
     { 0.55}
     
            
\def \flatfrequencyresponsezero 
     { 0.0}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,
             legend pos=north east,
             legend columns=3]
             
\addplot+[samples at = {0.00, 0.02, 0.04, 0.1, 		              
			  0.2, 0.3, 0.45, 0.6, 0.79, 1.03, 1.57}, 
          color = blue!60, 
          ycomb, 
          mark=otimes*, 
          mark options={blue!60}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {0.04, 0.175, 0.155, 0.34, 0.355, 
              0.66, 0.72, 1.17, 1.4}, 
          color = mygreen!60, 
          ycomb, 
          mark=otimes*, 
          mark options={mygreen!60}]
         {\flatfrequencyresponse};
         
         
\addplot+[samples at = {2.1}, 
          mark=*, 
          mark options={black, fill=white}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {2.1}, 
          mark=*, 
          mark options={black}]
         {\flatfrequencyresponsezero};

         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=0:2.1, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponse};
         
\addplot[ domain=2.1:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponsezero};
         

         


\end{axis}

\end{tikzpicture}

}


==> figures/figures/1030/49_high_pass_filter_eig__1_.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}
\def \unit {\thisplotscale cm}
       
\def \flatfrequencyresponse 
     { 0.55}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,
             legend pos=north east,
             legend columns=3]

\addplot+[samples at = {0.00, 0.02, 0.04, 0.1, 		              
			  0.2, 0.3, 0.45, 0.6, 0.79, 1.03, 1.57, 
              2.63, 3, 4.24, 5.51, 6.72, 7.6}, 
          color = blue!60, 
          ycomb, 
          mark=otimes*, 
          mark options={blue!60}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {0.04, 0.175, 0.155, 0.34, 0.355, 
              0.66, 0.72, 1.17, 1.4, 2.5, 3.13, 4.13, 
              5.68, 6.87, 7.8}, 
          color = mygreen!60, 
          ycomb, 
          mark=otimes*, 
          mark options={mygreen!60}]
         {\flatfrequencyresponse};
         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=0:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\flatfrequencyresponse};

%   \addlegendentry{\scriptsize $\bbW$}
%   \addlegendentry{\scriptsize $\bbG_n$}

\end{axis}

\end{tikzpicture}

}


==> figures/figures/1030/63_variable_band_filter.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}

\def \frequencyresponse 
     { 0.1*exp(-(1*(x-4.3))^2) 
       + 0.25*exp(-(2*(x-4.5))^2) 
       + 0.37*exp(-(1.3*(x-6.5))^2) 
       + 0.55}
       
\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 enlarge x limits = false,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,            					
             legend pos=north east,
             legend columns=3]
         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=0:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\frequencyresponse};

\end{axis}

\end{tikzpicture}

}



==> figures/figures/1030/66_variable_band_filter_graphon_eig.tex <==
%!TEX root = ../../../lecture_10_compile_handout/lecture_10_handout.tex
%!TEX root = ../../../lecture_10_compile_presentation/lecture_10_presentation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   CONTROL OF FIGURE SIZE AND PLOT RANGE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot scale. 
% 
\def \figurewidth   {12 cm}
\def \figureheight  { 3 cm}
\def \unit          { 1 cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Control plot range
% 
\def \xmin {-1} \def \xmax {1}
\def \ymin { 0} \def \ymax {1}
\def \yaxispad {0.05 }
\def \xaxispad {0.1 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   BEGIN FIGURE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\fontsize{7}{7}\selectfont


\pgfplotsset{xtick style={draw=none}}
\pgfplotsset{ytick style={draw=none}}

\def \thisplotscale {3.4}

\def \frequencyresponse 
     { 0.1*exp(-(1*(x-4.3))^2) 
       + 0.25*exp(-(2*(x-4.5))^2) 
       + 0.37*exp(-(1.3*(x-6.5))^2) 
       + 0.55}
       
\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\begin{axis}[scale only axis,
			 enlarge x limits = false,
			 width   = \figurewidth,
             height  = \figureheight,
             xmin = 0, xmax=8,
             xtick = {0, 2.1, 8},
             xticklabels = {\black{\footnotesize $0$},
             				\black\footnotesize {$c$}, 
                            \black{\footnotesize $1$}},
             ymin = -0, ymax = 1.15,
             ytick = {2},
             typeset ticklabels with strut,            					
             legend pos=north east,
             legend columns=3]

\addplot+[samples at = {0.00, 0.02, 0.04, 0.1, 		              
			  0.2, 0.3, 0.45, 0.6, 0.79, 1.03, 1.57, 
              2.63, 3, 4.24, 5.51, 6.72, 7.6}, 
          color = blue!60, 
          ycomb, 
          mark=otimes*, 
          mark options={blue!60}]
         {\frequencyresponse};
         
\addplot+[samples at = {0.04, 0.175, 0.155, 0.34, 0.355, 
              0.66, 0.72, 1.17, 1.4, 2.5, 3.13, 4.13, 
              5.68, 6.87, 7.8}, 
          color = mygreen!60, 
          ycomb, 
          mark=otimes*, 
          mark options={mygreen!60}]
         {\frequencyresponse};
         
\addplot+[samples at = {2.1}, 
          color = black!80, 
          dashed,
          ycomb,
          mark=none]
         {1.2};

\addplot[ domain=0:8, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\frequencyresponse};

\end{axis}

\end{tikzpicture}

}



==> figures/figures/macros/0_annotate_plot.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   % Annotate the graph with coordinates given 
      
   % Factor for translating plot coordinates into figure coordinates 
   \def \xfactor {\figurewidth  / \xmax}
   \def \yfactor {\figureheight / \ymax}

   % Annotate axis
   \node at (\xmax*\xfactor - \xmin*\xfactor, -\ydeltaskip*\yfactor) 
            [anchor = south west] 
            {$\lam_{\phantom{1}}$};

   \node at (\xmin*\xfactor, -0.14*\yfactor) 
            [anchor = south east] 
            {$\phantom{\lam_{\phantom{1}}}$};


   \node at (\xmin*\xfactor, \ymax*\yfactor) 
            [anchor = east] 
            {$\tdh(\lam)~$};

   \node at (\xmax*\xfactor - \xmin*\xfactor, \ymax*\yfactor) 
            [anchor = west] 
            {$\phantom{~{\tdh(\lam)}}$};


            
   % First three annotations. Associated with one signal
   \node at (\annotatedone*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationone};

   \node at (\annotatedtwo*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationtwo};

   \node at (\annotatedthree*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationthree};

   % Next three annotations. Associated with another signal
   \node at (\annotatedfour*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationfour};

   \node at (\annotatedfive*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationfive};

   \node at (\annotatedsix*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationsix};
   








==> figures/figures/macros/0_annotate_plot_no_axes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   % Annotate the graph with coordinates given 
      
   % Factor for translating plot coordinates into figure coordinates 
   \def \xfactor {\figurewidth  / \xmax}
   \def \yfactor {\figureheight / \ymax}

            
   % First three annotations. Associated with one signal
   \node at (\annotatedone*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationone};

   \node at (\annotatedtwo*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationtwo};

   \node at (\annotatedthree*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationthree};

   % Next three annotations. Associated with another signal
   \node at (\annotatedfour*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationfour};

   \node at (\annotatedfive*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationfive};

   \node at (\annotatedsix*\xfactor - \xmin*\xfactor , -\ydeltaskip*\yfactor) 
            [anchor = south] 
            {\annotationsix};
   








==> figures/figures/macros/0_draw_filter.tex <==
% Plot filter with a black thick line  

\addplot[ domain     = \xmin:\xmax,
          samples    = 150, 
          color      = black!99,
          line width = 1.2]
          { \filter };



==> figures/figures/macros/0_draw_gaussian_macro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Code for drawing Gaussian filter
% 
\newcommand{\drawgaussian}[7]
{
   \def \filter { ( \height*exp(-(1/\width*(x-\center))^2) ) }
   \def \center {#1}
   \def \width  {#2}
   \def \height {#3}

   \def \xminhere   {#4}
   \def \xmaxhere   {#5}

   % Draw filter Three
   \addplot[ domain     = \center-3.0*\width:\center + 3.0*\width, 
             samples    = 80, 
             color      = #6,
             line width = #7]
           { \filter };

   \addplot[ domain     = \xminhere:\center-3.0*\width, 
             samples    = 2, 
             color      = #6,
             line width = #7]
           { 0 };
   
   \addplot[ domain     = \center+3.0*\width:\xmaxhere, 
             samples    = 2, 
             color      = #6,
             line width = #7]
           { 0 };
}


==> figures/figures/macros/0_draw_gft_blue.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Plot GFT input and GFT ouptut at given spikes

   % Plot input spikes. Make them all of height 1
   \addplot+[ samples at   = \spikes, 
              ycomb, 
              mark         = otimes*, 
              color        =  blue!20, 
              mark options = {blue!20}
            ]
            { \ymax };

   %Plot frequency response spikes
   \addplot+[ samples at   = \spikes, 
              solid, 
              ycomb, 
              mark         = otimes*, 
              line width   = 1.2,              
              color        =  blue!60, 
              mark options = {blue!60}
            ]
            { \GFT*\filter};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   % Annotate the graph with three coordinates given 
   
   % Factor for translating plot coordinates into figure coordinates 
   \def \xfactor {\figurewidth  / \xmax}
   \def \yfactor {\figureheight / \ymax}

   % First three annotations. Associated with one signal
   \node at (\annotatedone*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationone};

   \node at (\annotatedtwo*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationtwo};

   \node at (\annotatedthree*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationthree};








==> figures/figures/macros/0_draw_gft_mygreen.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Plot GFT input and GFT ouptut at given spikes

   % Plot input spikes. Make them all of height 1
   \addplot+[ samples at   = \spikes, 
              ycomb, 
              mark         = otimes*, 
              color        =  mygreen!20, 
              mark options = {mygreen!20}
            ]
            { \ymax };

   %Plot frequency response spikes
   \addplot+[ samples at   = \spikes, 
              solid, 
              ycomb, 
              mark         = otimes*, 
              line width   = 1.2,              
              color        =  mygreen!60, 
              mark options = {mygreen!60}
            ]
            { \GFT*\filter};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   % Annotate the graph with three coordinates given 
   
   % Factor for translating plot coordinates into figure coordinates 
   \def \xfactor {\figurewidth  / \xmax}
   \def \yfactor {\figureheight / \ymax}

   % First three annotations. Associated with one signal
   \node at (\annotatedone*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationone};

   \node at (\annotatedtwo*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationtwo};

   \node at (\annotatedthree*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationthree};








==> figures/figures/macros/0_draw_gft_red.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Plot GFT input and GFT ouptut at given spikes

   % Plot input spikes. Make them all of height 1
   \addplot+[ samples at   = \spikes, 
              ycomb, 
              mark         = otimes*, 
              color        =  red!20, 
              mark options = {red!20}
            ]
            { \ymax };

   %Plot frequency response spikes
   \addplot+[ samples at   = \spikes, 
              solid, 
              ycomb, 
              mark         = otimes*, 
              line width   = 1.2,              
              color        =  red!60, 
              mark options = {red!60}
            ]
            { \GFT*\filter};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   % Annotate the graph with three coordinates given 
   
   % Factor for translating plot coordinates into figure coordinates 
   \def \xfactor {\figurewidth  / \xmax}
   \def \yfactor {\figureheight / \ymax}

   % First three annotations. Associated with one signal
   \node at (\annotatedone*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationone};

   \node at (\annotatedtwo*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationtwo};

   \node at (\annotatedthree*\xfactor, -0.14*\yfactor) 
            [anchor = south] 
            {\annotationthree};








==> figures/figures/macros/0_draw_shade.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macro to draw shadings in the background to highlight 
% eigenvalues that are moving 
 
   \newcommand{\drawshade}[3]
   {
      \path [fill = #3] 
            ( #1*\xfactor - \xmin*\xfactor - 5.0, 0.0*\yfactor) rectangle 
            ( #2*\xfactor - \xmin*\xfactor + 5.0, 1.0*\yfactor);
   }


